Entanglement-Efficient Distribution of Quantum Circuits over Large-Scale Quantum Networks

Quantum computers face inherent scaling challenges, a fact that necessitates investigation of distributed quantum computing systems, whereby scaling is achieved through interconnection of smaller quantum processing units. However, connecting large numbers of QPUs will eventually result in connectivity constraints at the network level, where the difficulty of entanglement sharing increases with network path lengths. This increases the complexity of the quantum circuit partitioning problem, since the cost of generating entanglement between end nodes varies with network topologies and existing links. We address this challenge using a simple modification to existing partitioning schemes designed for all-to-all connected networks, that efficiently accounts for both of these factors. We investigate the performance in terms of entanglement requirements and optimisation time of various quantum circuits over different network topologies, achieving lower entanglement costs in the majority of cases than state-of-the-art methods. We provide techniques for scaling to large-scale quantum networks employing both network and problem coarsening. We show that coarsened methods can achieve improved solution quality in most cases with significantly lower run-times than direct partitioning methods.

==> PGF/CP/Combined/Combined_CP_2-12_wrapper.tex <==
\begin{tikzpicture}
    % Define positioning
    \node[anchor=south west] (linear_cost) at (0,3) {%
        \resizebox{0.45\textwidth}{!}{\input{PGF/CP/NetCoarse/new_results/figure_128_linear_nolabel.tex}}%
    };
    
    \node[anchor=south west] (grid_cost) at (0.5\textwidth,3) {%
        \resizebox{0.45\textwidth}{!}{\input{PGF/CP/NetCoarse/new_results/figure_128_grid_nolabel.tex}}%
    };
    
    \node[anchor=south west] (linear_time) at (0,0) {%
        \resizebox{0.45\textwidth}{!}{\input{PGF/CP/NetCoarse/new_results/figure_128_linear_time_nolabel.tex}}%
    };
    
    \node[anchor=south west] (grid_time) at (0.5\textwidth,0) {%
        \resizebox{0.45\textwidth}{!}{\input{PGF/CP/NetCoarse/new_results/figure_128_grid_time_nolabel.tex}}%
    };
    
    % Add shared axis labels
    \node[rotate=90] at (-0.8,3.75) {\footnotesize Entanglement cost};
    \node[rotate=90] at (-0.8,1.5) {\footnotesize Time taken (s)};
    
    % Add titles
    \node at (0.225\textwidth,6.2) {\footnotesize Linear 128-qubit};
    \node at (0.725\textwidth,6.2) {\footnotesize Grid 128-qubit};
    
\end{tikzpicture}


==> PGF/CP/NetCoarse/combined_nets_copy.tex <==
\usetikzlibrary{patterns}
\begin{tikzpicture}
    \begin{axis}[
      width=\columnwidth,
      height=0.75\columnwidth,
        ybar,                     % Use bars
        bar width=2.5pt,         % Control bar thickness
        symbolic x coords={4,16,64},
        unbounded coords=discard, % Discard unbound coords
        xtick={4,16,64},
        enlarge x limits=0.1,    % A bit of horizontal padding
        ymin=0, ymax=200000,        % Pick whichever max fits both data sets
        xlabel={Number of QPUs},
        ylabel={Entanglement cost},
        grid=minor,
        minor grid style={line width=0.5pt, draw=gray!60, densely dotted},
        major grid style={dotted, draw=gray!70},
        scaled y ticks = base 10:-2,
        % We'll manage the legend ourselves to avoid duplication
        legend style={
          at={(1.0,1.1)},
          anchor=south,
          legend columns=4,
       },
        error bars/y dir=both,
        error bars/y explicit,
        error bars/error mark options={
            rotate=90,
            mark size=1pt
        }
    ]
    
    % -- METHOD 1: FGP-rOEE -----------------------------------
    % 2-partitions
    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Linear/NetCoarse_CP_2-12.dat}\dataLinear
    \addplot+ [
      color=blue,
      fill opacity=0.3,
      bar shift=-9pt,
    ] table [
      x=num_partitions,
      y=r_cost_mean,
      y error plus expr=\thisrow{r_cost_upper}-\thisrow{r_cost_mean},
      y error minus expr=\thisrow{r_cost_mean}-\thisrow{r_cost_lower},
    ] {\dataLinear};

    \addlegendentry{Linear Coarsened}

    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Grid/NetCoarse_CP_2-12.dat}\dataGrid
    \addplot+ [
      color=red,
      fill opacity=0.3,
      bar shift=3pt,
    ] table [
      x=num_partitions,
      y=r_cost_mean,
      y error plus expr=\thisrow{r_cost_upper}-\thisrow{r_cost_mean},
      y error minus expr=\thisrow{r_cost_mean}-\thisrow{r_cost_lower},
    ] {\dataGrid};

    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Comparison/Linear/NetCoarse_CP_2-12.dat}\dataLinDirect
    % \addplot+ [
    %   color=orange,
    %   fill opacity=0.3,
    %   bar shift=-20pt,
  
    % ] table [
    %   x=num_partitions,
    %   y=r_cost_mean,
    %   y error plus expr=\thisrow{r_cost_upper}-\thisrow{r_cost_mean},
    %   y error minus expr=\thisrow{r_cost_mean}-\thisrow{r_cost_lower},
    % ] {\dataLinDirect};

    \addlegendentry{Grid Coarsened}

    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Comparison/Linear/NetCoarse_CP_2-12.dat}\dataLinDirect
    \addplot+ [
      color=orange,
      fill opacity=0.3,
      bar shift=-3pt,
    ] table [
      x=num_partitions,
      y=r_cost_mean,
      y error plus expr=\thisrow{r_cost_upper}-\thisrow{r_cost_mean},
      y error minus expr=\thisrow{r_cost_mean}-\thisrow{r_cost_lower},
    ] {\dataLinDirect};

    \addlegendentry{Direct Linear}

    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Comparison/Grid/NetCoarse_CP_2-12.dat}\dataGridDirect
    \addplot+ [
      color=teal,
      fill opacity=0.3,
      bar shift=1000pt,
    ] table [
      x=num_partitions,
      y=r_cost_mean,
      y error plus expr=\thisrow{r_cost_upper}-\thisrow{r_cost_mean},
      y error minus expr=\thisrow{r_cost_mean}-\thisrow{r_cost_lower},
    ] {\dataGridDirect};

    % \addlegendentry{Direct Grid}


    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Comparison/Grid/NetCoarse_CP_2-12.dat}\dataGridDirect
    \addplot+ [
      color=teal,
      fill opacity=0.3,
      bar shift=9pt,
    ] table [
      x=num_partitions,
      y=r_cost_mean,
      y error plus expr=\thisrow{r_cost_upper}-\thisrow{r_cost_mean},
      y error minus expr=\thisrow{r_cost_mean}-\thisrow{r_cost_lower},
    ] {\dataGridDirect};

    \addlegendentry{Direct Grid}



    
    % We only want ONE legend entry for FGP-rOEE overall:
    
    % % 4-partitions
    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/Data/FGP/QFT/QFT_4_cost.dat}\dataFGPfour
    % \addplot+ [
    %   color=one,
    %   fill opacity=0.3,
    %   pattern=north east lines,   % no pattern => "4 partitions"
    %   bar shift=3pt,
    %   forget plot,    % DO NOT add a second FGP legend entry
    % ] table [
    %   x=num_qubits,
    %   y=fgp_mean,
    %   y error plus expr=\thisrow{fgp_max}-\thisrow{fgp_mean},
    %   y error minus expr=\thisrow{fgp_mean}-\thisrow{fgp_min},
    % ] {\dataFGPfour};
    
    % \addlegendentry{FGP-rOEE}
    
    % % -- METHOD 2: MLFM-R --------------------------------------
    % % 2-partitions
    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/Data/FM/QFT/QFT_2_cost.dat}\dataFMtwo
    % \addplot+ [
    %   color=teal,
    %   fill opacity=0.3,
    %   bar shift=-6pt,
    % ] table [
    %   x=num_qubits,
    %   y=r_mean,
    %   y error plus expr=\thisrow{r_max}-\thisrow{r_mean},
    %   y error minus expr=\thisrow{r_mean}-\thisrow{r_min},
    % ] {\dataFMtwo};
    
    
    
    % % 4-partitions
    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/Data/FM/QFT/QFT_4_cost.dat}\dataFMfour
    % \addplot+ [
    %   color=teal,
    %   fill opacity=0.3,
    %   pattern=north east lines,
    %   bar shift=6pt,
    %   forget plot,
    % ] table [
    %   x=num_qubits,
    %   y=r_mean,
    %   y error plus expr=\thisrow{r_max}-\thisrow{r_mean},
    %   y error minus expr=\thisrow{r_mean}-\thisrow{r_min},
    % ] {\dataFMfour};
    
    % \addlegendentry{MLFM-R}
    
    % % -- METHOD 3: Pytket PE -----------------------------------
    % % 2-partitions
    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/Data/Tket/PE/QFT/QFT_2_cost.dat}\dataTKtwo
    % \addplot+ [
    %   color=three,
    %   fill opacity=0.3,
    %   bar shift=-3pt,
    % ] table [
    %   x=num_qubits,
    %   y=embed_mean,
    %   y error plus expr=\thisrow{embed_max}-\thisrow{embed_mean},
    %   y error minus expr=\thisrow{embed_mean}-\thisrow{embed_min},
    % ] {\dataTKtwo};
    
    % \addlegendentry{Pytket PE}
    
    
    % \pgfplotstableread[
    %   col sep=space,
    %   header=has colnames
    % ]{PGF/Data/Tket/PE/QFT/QFT_4_cost.dat}\datatable
    % \addplot+ [
    %   color=gray,
    % fill opacity=.3,
    % bar shift = -10000pt,
    % ]
    % table [
    %   x=num_qubits,
    %   y=,
    % ] {\datatable};
    
    
    
    % % 4-partitions
    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Grid/NetCoarse_CP_2-12.dat}\dataTKfour
    % \addplot+ [
    %   color=three,
    %   fill opacity=0.3,
    %   pattern=north east lines,
    %   bar shift=9pt,
    %   forget plot,
    % ] table [
    %   x=num_qubits,
    %   y=embed_mean,
    %   y error plus expr=\thisrow{embed_max}-\thisrow{embed_mean},
    %   y error minus expr=\thisrow{embed_mean}-\thisrow{embed_min},
    % ] {\dataTKfour};
    
    % --- Now add *just two* extra legend entries to show patterns ---
    % 1) "2 partitions" => (pattern)
    
    % \addlegendimage{area legend, fill=gray, pattern = north east lines, fill opacity=0.3}
    % \addlegendentry{2 QPU}
    
    % % 2) "4 partitions" => (no pattern)
    % \addlegendimage{area legend, pattern=north east lines, fill=gray, fill opacity=0.3}
    % \addlegendentry{4 QPU}
    
    \end{axis}
    
    % \node at (4.25,3.8) {%
    %   \begin{tikzpicture}[font=\footnotesize]
    %     % 1) A small blue box at (0,0):
    %     \draw[fill=gray] (0,0) rectangle (0.3,0.3);
    %     % Text label to its right
    %     \node[anchor=west] at (0.4,0.15) {2 QPUs};
    
    %     % 2) A red patterned box lower down at (0,-0.5):
    %     \draw[fill=gray, pattern=north east lines] (0,-0.5) rectangle (0.3,-0.2);
    %     % Text label to its right
    %     \node[anchor=west] at (0.4,-0.35) {4 QPUs};
    
    %     % You can add more entries as needed, each with its own position
    %   \end{tikzpicture}%
    % };
    \end{tikzpicture}
    

==> PGF/CP/NetCoarse/combined_nets_new.tex <==
\usetikzlibrary{patterns}
\begin{tikzpicture}
    \begin{axis}[
      width=\columnwidth,
      height=0.75\columnwidth,
        ybar,                     % Use bars
        bar width=2.5pt,         % Control bar thickness
        symbolic x coords={4,16,64},
        unbounded coords=discard, % Discard unbound coords
        xtick={4,16,64},
        enlarge x limits=0.1,    % A bit of horizontal padding
        ymin=0, ymax=200000,        % Pick whichever max fits both data sets
        xlabel={Number of QPUs},
        ylabel={Entanglement cost},
        grid=minor,
        minor grid style={line width=0.5pt, draw=gray!60, densely dotted},
        major grid style={dotted, draw=gray!70},
        scaled y ticks = base 10:-2,
        % We'll manage the legend ourselves to avoid duplication
        legend style={
          at={(1.0,1.1)},
          anchor=south,
          legend columns=4,
       },
        error bars/y dir=both,
        error bars/y explicit,
        error bars/error mark options={
            rotate=90,
            mark size=1pt
        }
    ]
    
    % -- METHOD 1: FGP-rOEE -----------------------------------
    % 2-partitions
    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Linear/NetCoarse_CP_2-12.dat}\dataLinear
    \addplot+ [
      color=blue,
      fill opacity=0.3,
      bar shift=-9pt,
    ] table [
      x=num_partitions,
      y=r_cost_mean,
      y error plus expr=\thisrow{r_cost_upper}-\thisrow{r_cost_mean},
      y error minus expr=\thisrow{r_cost_mean}-\thisrow{r_cost_lower},
    ] {\dataLinear};

    \addlegendentry{Linear Coarsened}

    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Grid/NetCoarse_CP_2-12.dat}\dataGrid
    \addplot+ [
      color=red,
      fill opacity=0.3,
      bar shift=3pt,
    ] table [
      x=num_partitions,
      y=r_cost_mean,
      y error plus expr=\thisrow{r_cost_upper}-\thisrow{r_cost_mean},
      y error minus expr=\thisrow{r_cost_mean}-\thisrow{r_cost_lower},
    ] {\dataGrid};

    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Comparison/Linear/NetCoarse_CP_2-12.dat}\dataLinDirect
    % \addplot+ [
    %   color=orange,
    %   fill opacity=0.3,
    %   bar shift=-20pt,
  
    % ] table [
    %   x=num_partitions,
    %   y=r_cost_mean,
    %   y error plus expr=\thisrow{r_cost_upper}-\thisrow{r_cost_mean},
    %   y error minus expr=\thisrow{r_cost_mean}-\thisrow{r_cost_lower},
    % ] {\dataLinDirect};

    \addlegendentry{Grid Coarsened}

    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Comparison/Linear/NetCoarse_CP_2-12.dat}\dataLinDirect
    \addplot+ [
      color=orange,
      fill opacity=0.3,
      bar shift=-3pt,
    ] table [
      x=num_partitions,
      y=r_cost_mean,
      y error plus expr=\thisrow{r_cost_upper}-\thisrow{r_cost_mean},
      y error minus expr=\thisrow{r_cost_mean}-\thisrow{r_cost_lower},
    ] {\dataLinDirect};

    \addlegendentry{Direct Linear}

    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Comparison/Grid/NetCoarse_CP_2-12.dat}\dataGridDirect
    \addplot+ [
      color=teal,
      fill opacity=0.3,
      bar shift=1000pt,
    ] table [
      x=num_partitions,
      y=r_cost_mean,
      y error plus expr=\thisrow{r_cost_upper}-\thisrow{r_cost_mean},
      y error minus expr=\thisrow{r_cost_mean}-\thisrow{r_cost_lower},
    ] {\dataGridDirect};

    % \addlegendentry{Direct Grid}


    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Comparison/Grid/NetCoarse_CP_2-12.dat}\dataGridDirect
    \addplot+ [
      color=teal,
      fill opacity=0.3,
      bar shift=9pt,
    ] table [
      x=num_partitions,
      y=r_cost_mean,
      y error plus expr=\thisrow{r_cost_upper}-\thisrow{r_cost_mean},
      y error minus expr=\thisrow{r_cost_mean}-\thisrow{r_cost_lower},
    ] {\dataGridDirect};

    \addlegendentry{Direct Grid}
    
    \end{axis}
    
    % \node at (4.25,3.8) {%
    %   \begin{tikzpicture}[font=\footnotesize]
    %     % 1) A small blue box at (0,0):
    %     \draw[fill=gray] (0,0) rectangle (0.3,0.3);
    %     % Text label to its right
    %     \node[anchor=west] at (0.4,0.15) {2 QPUs};
    
    %     % 2) A red patterned box lower down at (0,-0.5):
    %     \draw[fill=gray, pattern=north east lines] (0,-0.5) rectangle (0.3,-0.2);
    %     % Text label to its right
    %     \node[anchor=west] at (0.4,-0.35) {4 QPUs};
    
    %     % You can add more entries as needed, each with its own position
    %   \end{tikzpicture}%
    % };
    \end{tikzpicture}
    

==> PGF/CP/NetCoarse/combined_nets_time.tex <==
\usetikzlibrary{patterns}
\begin{tikzpicture}
    \begin{axis}[
      width=\columnwidth,
      height=0.75\columnwidth,
        ybar,                     % Use bars
        bar width=2.5pt,         % Control bar thickness
        symbolic x coords={4,16,64},
        unbounded coords=discard, % Discard unbound coords
        xtick={4,16,64},
        enlarge x limits=0.1,    % A bit of horizontal padding
        ymin=0, ymax=1200,        % Pick whichever max fits both data sets
        xlabel={Number of QPUs},
        ylabel={Time (s)},
        grid=minor,
        minor grid style={line width=0.5pt, draw=gray!60, densely dotted},
        major grid style={dotted, draw=gray!70},
        scaled y ticks = base 10:-2,
        % We'll manage the legend ourselves to avoid duplication
        legend style={
          at={(0.3,0.7)},
          anchor=south,
          legend columns=1,
       },
        error bars/y dir=both,
        error bars/y explicit,
        error bars/error mark options={
            rotate=90,
            mark size=1pt
        }
    ]
    
    % -- METHOD 1: FGP-rOEE -----------------------------------
    % 2-partitions
    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Linear/NetCoarse_CP_2-12.dat}\dataLinear
    \addplot+ [
      color=blue,
      fill opacity=0.3,
      bar shift=-9pt,
    ] table [
      x=num_partitions,
      y=time_r_mean,
      y error plus expr=\thisrow{time_r_upper}-\thisrow{time_r_mean},
      y error minus expr=\thisrow{time_r_mean}-\thisrow{time_r_lower},
    ] {\dataLinear};

    % \addlegendentry{Linear Coarsened}

    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Grid/NetCoarse_CP_2-12.dat}\dataGrid
    \addplot+ [
      color=red,
      fill opacity=0.3,
      bar shift=3pt,
    ] table [
      x=num_partitions,
      y=time_r_mean,
      y error plus expr=\thisrow{time_r_upper}-\thisrow{time_r_mean},
      y error minus expr=\thisrow{time_r_mean}-\thisrow{time_r_lower},
    ] {\dataGrid};


    % \addlegendentry{Grid Coarsened}

    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Comparison/Linear/NetCoarse_CP_2-12.dat}\dataLinDirect
    \addplot+ [
      color=orange,
      fill opacity=0.3,
      bar shift=-3pt,
    ] table [
      x=num_partitions,
      y=time_r_mean,
      y error plus expr=\thisrow{time_r_upper}-\thisrow{time_r_mean},
      y error minus expr=\thisrow{time_r_mean}-\thisrow{time_r_lower},
    ] {\dataLinDirect};

    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Comparison/Linear/NetCoarse_CP_2-12.dat}\dataLinDirect
    % \addplot+ [
    %   color=orange,
    %   fill opacity=0.3,
    %   bar shift=-20pt,
  
    % ] table [
    %   x=num_partitions,
    %   y=_r_mean,
    %   y error plus expr=\thisrow{time_r_upper}-\thisrow{time_r_mean},
    %   y error minus expr=\thisrow{time_r_mean}-\thisrow{time_r_lower},

    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Comparison/Grid/NetCoarse_CP_2-12.dat}\dataGridDirect
    \addplot+ [
      color=white,
      fill opacity=0.3,
      bar shift=100pt,
    ] table [
      x=num_partitions,
      y=time_r_mean,
      y error plus expr=\thisrow{time_r_upper}-\thisrow{time_r_mean},
      y error minus expr=\thisrow{time_r_mean}-\thisrow{time_r_lower},
    ] {\dataGridDirect};

    \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Comparison/Grid/NetCoarse_CP_2-12.dat}\dataGridDirect
    \addplot+ [
      color=teal,
      fill opacity=0.3,
      bar shift=9pt,
    ] table [
      x=num_partitions,
      y=time_r_mean,
      y error plus expr=\thisrow{time_r_upper}-\thisrow{time_r_mean},
      y error minus expr=\thisrow{time_r_mean}-\thisrow{time_r_lower},
    ] {\dataGridDirect};


    
    % We only want ONE legend entry for FGP-rOEE overall:
    
    % % 4-partitions
    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/Data/FGP/QFT/QFT_4_cost.dat}\dataFGPfour
    % \addplot+ [
    %   color=one,
    %   fill opacity=0.3,
    %   pattern=north east lines,   % no pattern => "4 partitions"
    %   bar shift=3pt,
    %   forget plot,    % DO NOT add a second FGP legend entry
    % ] table [
    %   x=num_qubits,
    %   y=fgp_mean,
    %   y error plus expr=\thisrow{fgp_max}-\thisrow{fgp_mean},
    %   y error minus expr=\thisrow{fgp_mean}-\thisrow{fgp_min},
    % ] {\dataFGPfour};
    
    % \addlegendentry{FGP-rOEE}
    
    % % -- METHOD 2: MLFM-R --------------------------------------
    % % 2-partitions
    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/Data/FM/QFT/QFT_2_cost.dat}\dataFMtwo
    % \addplot+ [
    %   color=teal,
    %   fill opacity=0.3,
    %   bar shift=-6pt,
    % ] table [
    %   x=num_qubits,
    %   y=r_mean,
    %   y error plus expr=\thisrow{r_max}-\thisrow{r_mean},
    %   y error minus expr=\thisrow{r_mean}-\thisrow{r_min},
    % ] {\dataFMtwo};
    
    
    
    % % 4-partitions
    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/Data/FM/QFT/QFT_4_cost.dat}\dataFMfour
    % \addplot+ [
    %   color=teal,
    %   fill opacity=0.3,
    %   pattern=north east lines,
    %   bar shift=6pt,
    %   forget plot,
    % ] table [
    %   x=num_qubits,
    %   y=r_mean,
    %   y error plus expr=\thisrow{r_max}-\thisrow{r_mean},
    %   y error minus expr=\thisrow{r_mean}-\thisrow{r_min},
    % ] {\dataFMfour};
    
    % \addlegendentry{MLFM-R}
    
    % % -- METHOD 3: Pytket PE -----------------------------------
    % % 2-partitions
    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/Data/Tket/PE/QFT/QFT_2_cost.dat}\dataTKtwo
    % \addplot+ [
    %   color=three,
    %   fill opacity=0.3,
    %   bar shift=-3pt,
    % ] table [
    %   x=num_qubits,
    %   y=embed_mean,
    %   y error plus expr=\thisrow{embed_max}-\thisrow{embed_mean},
    %   y error minus expr=\thisrow{embed_mean}-\thisrow{embed_min},
    % ] {\dataTKtwo};
    
    % \addlegendentry{Pytket PE}
    
    
    % \pgfplotstableread[
    %   col sep=space,
    %   header=has colnames
    % ]{PGF/Data/Tket/PE/QFT/QFT_4_cost.dat}\datatable
    % \addplot+ [
    %   color=gray,
    % fill opacity=.3,
    % bar shift = -10000pt,
    % ]
    % table [
    %   x=num_qubits,
    %   y=,
    % ] {\datatable};
    
    
    
    % % 4-partitions
    % \pgfplotstableread[col sep=space,header=has colnames]{PGF/CP/NetCoarse/Grid/NetCoarse_CP_2-12.dat}\dataTKfour
    % \addplot+ [
    %   color=three,
    %   fill opacity=0.3,
    %   pattern=north east lines,
    %   bar shift=9pt,
    %   forget plot,
    % ] table [
    %   x=num_qubits,
    %   y=embed_mean,
    %   y error plus expr=\thisrow{embed_max}-\thisrow{embed_mean},
    %   y error minus expr=\thisrow{embed_mean}-\thisrow{embed_min},
    % ] {\dataTKfour};
    
    % --- Now add *just two* extra legend entries to show patterns ---
    % 1) "2 partitions" => (pattern)
    
    % \addlegendimage{area legend, fill=gray, pattern = north east lines, fill opacity=0.3}
    % \addlegendentry{2 QPU}
    
    % % 2) "4 partitions" => (no pattern)
    % \addlegendimage{area legend, pattern=north east lines, fill=gray, fill opacity=0.3}
    % \addlegendentry{4 QPU}
    
    \end{axis}
    
    % \node at (4.25,3.8) {%
    %   \begin{tikzpicture}[font=\footnotesize]
    %     % 1) A small blue box at (0,0):
    %     \draw[fill=gray] (0,0) rectangle (0.3,0.3);
    %     % Text label to its right
    %     \node[anchor=west] at (0.4,0.15) {2 QPUs};
    
    %     % 2) A red patterned box lower down at (0,-0.5):
    %     \draw[fill=gray, pattern=north east lines] (0,-0.5) rectangle (0.3,-0.2);
    %     % Text label to its right
    %     \node[anchor=west] at (0.4,-0.35) {4 QPUs};
    
    %     % You can add more entries as needed, each with its own position
    %   \end{tikzpicture}%
    % };
    \end{tikzpicture}
    
